Parallel simulation of two--dimensional Ising models using Probabilistic Cellular Automata

We perform a numerical investigation of the \emph{shaken dynamics}, a parallel Markovian dynamics for spin systems with local interaction and whose transition probabilities depend on two parameters, $q$ and $J$, that tune the geometry of the underlying lattice. We determine a phase transition curve, in the $(q, J)$ plane, separating the disordered phase from the ordered one, study the mixing time of the Markov chain and evaluate the spin-spin correlations as $q$ and $J$ vary. Further, we investigate the relation between the equilibrium measure of the shaken dynamics and the Gibbs measure for the Ising model. Two different approaches are considered for the implementation of the dynamics: a multicore CPU approach, with code written in Julia and a GPU approach with code written in CUDA.

==> Figure/shakenLatticeHexagon.tex <==
%auto-ignore

\begin{tikzpicture}

	\tikzmath{
		\xs=0.6;
		\ys=0.6;
	}

	\draw[step=2cm,gray,very thin] (0.1,0.1) grid (9.9,9.9);
	\draw[step=2cm,gray,very thin, dashed, shift={(-\xs, -\ys)}] (0.1,0.1) grid (9.9,9.9);

	\foreach \x in {0, 2, 4, 6, 8}
		\foreach \y in {0, 2, 4, 6, 8}
			{\draw[red] (\x,\y) -- (\x-\xs, \y-\ys);
			 \draw[red] (\x,\y) -- (\x-\xs, \y+2-\ys);
			 \draw[red] (\x,\y) -- (\x+2-\xs, \y-\ys);
			}

		\path(4,4) -- node [anchor=south east]{$q$} (4-\xs, 4-\xs);
		\path(2,4) -- node [anchor=north east, pos=0.6]{$J$} (4-\xs, 4-\ys);
		\path(4,2) -- node [anchor=north east, pos=0.6]{$J$} (4-\xs, 4-\ys);

		\path(8,8) -- node [color=black, anchor=south]{$\Lambda_\sigma$} (10,8);
		\path[xshift=-\xs cm, yshift=-\ys cm](8,8) -- node [color=black, anchor=north]{$\Lambda_\tau$} (10,8);

\end{tikzpicture}

